Differential Motion Evolution for Fine-Grained Motion Deformation in Unsupervised Image Animation

Image animation is the task of transferring the motion of a driving video to a given object in a source image. While great progress has recently been made in unsupervised motion transfer, requiring no labeled data or domain priors, many current unsupervised approaches still struggle to capture the motion deformations when large motion/view discrepancies occur between the source and driving domains. Under such conditions, there is simply not enough information to capture the motion field properly. We introduce DiME (Differential Motion Evolution), an end-to-end unsupervised motion transfer framework integrating differential refinement for motion estimation. Key findings are twofold: (1) by capturing the motion transfer with an ordinary differential equation (ODE), it helps to regularize the motion field, and (2) by utilizing the source image itself, we are able to inpaint occluded/missing regions arising from large motion changes. Additionally, we also propose a natural extension to the ODE idea, which is that DiME can easily leverage multiple different views of the source object whenever they are available by modeling an ODE per view. Extensive experiments across 9 benchmarks show DiME outperforms the state-of-the-arts by a significant margin and generalizes much better to unseen objects.

==> sub/tab/archive/tab_all.tex <==

\begin{table}[!th] 
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{1.0\linewidth}{!}{
%\hspace{-1cm}
(a)
\begin{tabular}{cccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

{\textbf{\textit{Dataset}}} & {\textbf{\textit{Method}}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} \\

\specialrule{.08em}{.05em}{.05em}
%\hlineå



\multicolumn{1}{c}{\multirow{4}{*}{\shortstack{\texttt{VoxCeleb}\\(507)}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.047  & 0.14  & 50.96 & (0.84) 0.75 & 22.74 & 2.29  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.044  & 0.13  & 50.69 & (0.86) 0.77 & 23.18 & 2.15  \\ 

& \textit{f-v2v} \cite{Wang_2021_CVPR} & 0.042 & N/A  & 69.13 & (0.85) 0.80 & 24.37 & 2.07  \\ 

& \textit{Ours} & {\bf{0.027}}   & {\bf{0.071}}  & {\bf{25.43}} & ({\bf{0.93}}) {\bf{0.86}} & {\bf{26.20}} & {\bf{1.90}}    \\ 
  
%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\td{\texttt{DFDC}}\\\td{(200)}}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} &  &  &   &   &   &    \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} &  &  &   &   &   &    \\  

& \textit{Ours} &  &  &   &   &   &    \\ 
  

%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Nemo}\\(124)}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.0139  & 0.034 & 19.60 & (0.96) 0.95 & 32.90 & 1.17   \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.0169 & 0.041 & 30.09 & (0.95) 0.93 & 30.55 & 1.32 \\  

& \textit{Ours} & {\bf{0.0061}} & {\bf{0.013}} & {\bf{10.35}} & {\bf{0.99}} ({\bf{0.98}}) & {\bf{39.40}} & {\bf{0.87}}   \\ 

\specialrule{.15em}{.05em}{.05em} 
\end{tabular} 


}



\resizebox{1.0\linewidth}{!}{
(b)
\begin{tabular}{cccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

{\textbf{\textit{Dataset}}} & {\textbf{\textit{Method}}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} \\

\specialrule{.08em}{.05em}{.05em}
%\hlineå



\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Fashion}\\(100)}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.013 & 0.033 & 30.73 & (0.96) 0.93 & 27.06 & 1.09  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.015 & 0.040 & 37.99 & (0.95) 0.92 & 25.88 & 1.54  \\  

& \textit{Ours} & {\bf{0.010}} & {\bf{0.030}} & {\bf{22.25}} & ({\bf{0.95}}) {\bf{0.97}} & {\bf{26.95}} & {\bf{1.00}}    \\ 
  
%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\td{\texttt{AIST}}\\ \td{(200)}}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS}  &   &   &   &  &   &    \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} &   &   &   &  &   &    \\  

& \textit{Ours}  &   &   &   &  &   &    \\ 
  
%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Tai-Chi-HD}\\(87)}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS}  & 0.057 & 0.24 & 123.78 & (0.69) 0.64 & 20.45 & 9.69 \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.059 & 0.21 & 109.56 & (0.70) 0.57 & 20.31 & 7.30   \\  

& \textit{Ours}  & {\bf{0.035}} & {\bf{0.15}} & {\bf{76.41}} & ({\bf{0.83}}) {\bf{0.78}} & {\bf{23.08}} & {\bf{6.36}}  \\ 


\specialrule{.15em}{.05em}{.05em} 
\end{tabular} 


}


\resizebox{1.0\linewidth}{!}{
(c)
\begin{tabular}{ccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

 
%\cmidrule(lr){2-6}

{\textbf{\textit{Dataset}}} & {\textbf{\textit{Method}}} & {\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & {\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & {\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & {\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & {\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}}  \\

\specialrule{.08em}{.05em}{.05em}
%\hline

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Bair}\\(128)}}} & \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.030 & 0.067 & 107.70 & (0.91) 0.88 & 23.64  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.052 & 0.137 & 217.87 & (0.87) 0.76 & 19.75  \\ 

& \textit{Ours} & {\bf{0.018}} & {\bf{0.027}} & {\bf{96.91}} & {\bf{(0.97) 0.94}} & {\bf{27.75}}  \\ 


%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%
 
\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{MGif}\\(100)}}} & \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.033 & 0.112 & 154.88 & (0.87) 0.84 & 19.56  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.027 & 0.092 & 136.84 & (0.90) 0.85 & 20.22 \\ 

& \textit{Ours} & {\bf{0.021}} & {\bf{0.072}} & {\bf{117.74}} & {\bf{(0.92) 0.90}} & {\bf{21.34}} \\ 
  
\specialrule{.15em}{.05em}{.05em}
 
\end{tabular} 
}


\caption{Reconstruction results for FOMM \cite{Siarohin_2019_NeurIPS} (re-trained), Articulated Animation (AA) \cite{Siarohin_2021_CVPR} (re-trained), face-vid2vid (f-v2v) \cite{Wang_2021_CVPR} (reported) and our approach on (a) face datasets (\texttt{VoxCeleb}, \texttt{DFDC}, \texttt{Nemo}), (b) body datasets (\texttt{Fashion}, \texttt{AIST}, \texttt{Tai-Chi-HD}) and (c) robot (\texttt{Bair}) \& cartoon animals (\texttt{MGif}) datasets. Results are reported in mean format with best ones bolded. The number of reconstruction testing samples are listed in parentheses below each dataset name. $\downarrow$ ($\uparrow$) denotes that lower (higher) is better.  Our approach consistently achieves the best performance on \textit{all} metrics across \textit{all} eight datasets.
}
\label{tab: recon_all}
\end{table}

==> sub/tab/archive/tab_recon_bair_mgif.tex <==

\begin{table}[!th] 
\centering
\renewcommand{\arraystretch}{1.}

\resizebox{1.0\linewidth}{!}{
\begin{tabular}{ccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

 
%\cmidrule(lr){2-6}

Dataset & Method & {\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & {\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & {\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & {\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & {\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}}  \\

\specialrule{.15em}{.05em}{.05em}
%\hline

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Bair}\\(128)}}} & \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.030 & 0.067 & 107.70 & (0.91) 0.88 & 23.64  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.052 & 0.137 & 217.87 & (0.87) 0.76 & 19.75  \\ 

& \textit{Ours} & {\bf{0.018}} & {\bf{0.027}} & {\bf{96.91}} & {\bf{(0.97) 0.94}} & {\bf{27.75}}  \\ 


%%%%%%%%%%%
\specialrule{.08em}{.05em}{.05em}
%\hline
%%%%%%%%%%%
 
\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{MGif}\\(100)}}} & \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.033 & 0.112 & 154.88 & (0.87) 0.84 & 19.56  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.027 & 0.092 & 136.84 & (0.90) 0.85 & 20.22 \\ 

& \textit{Ours} & {\bf{0.021}} & {\bf{0.072}} & {\bf{117.74}} & {\bf{(0.92) 0.90}} & {\bf{21.34}} \\ 
  
\specialrule{.15em}{.05em}{.05em}


\end{tabular} 
}

\caption{Reconstruction results for FOMM \cite{Siarohin_2019_NeurIPS} (re-trained), Articulated Animation (AA) \cite{Siarohin_2021_CVPR} (re-trained) and our approach on robots (\texttt{Bair}) and cartoon animals (\texttt{MGif}) datasets. Best results are bolded. The number of testing samples are listed in parentheses under dataset names. $\downarrow$ ($\uparrow$) denotes that lower (higher) is better. }

\label{tab: recon_bair_mgif}
\end{table}

==> sub/tab/archive/tab_recon_body.tex <==

\begin{table}[!th] 
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{1.0\linewidth}{!}{\begin{tabular}{cccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

Dataset & Method & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} \\

\specialrule{.15em}{.05em}{.05em}
%\hlineå



\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Fashion}\\(100)}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.013 & 0.033 & 30.73 & (0.96) 0.93 & 27.06 & 1.09  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.015 & 0.040 & 37.99 & (0.95) 0.92 & 25.88 & 1.54  \\  

& \textit{Ours} & {\bf{0.010}} & {\bf{0.030}} & {\bf{22.25}} & ({\bf{0.95}}) {\bf{0.97}} & {\bf{26.95}} & {\bf{1.00}}    \\ 
  
%%%%%%%%%%%
\specialrule{.08em}{.05em}{.05em}
%\hline
%%%%%%%%%%% 

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\td{\texttt{AIST}}\\ \td{(200)}}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS}  &   &   &   &  &   &    \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} &   &   &   &  &   &    \\  

& \textit{Ours}  &   &   &   &  &   &    \\ 
  
%%%%%%%%%%%
\specialrule{.08em}{.05em}{.05em}
%\hline
%%%%%%%%%%% 

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Tai-Chi-HD}\\(87)}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS}  & 0.057 & 0.24 & 123.78 & (0.69) 0.64 & 20.45 & 9.69 \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.059 & 0.21 & 109.56 & (0.70) 0.57 & 20.31 & 7.30   \\  

& \textit{Ours}  & {\bf{0.035}} & {\bf{0.15}} & {\bf{76.41}} & ({\bf{0.83}}) {\bf{0.78}} & {\bf{23.08}} & {\bf{6.36}}  \\ 


\specialrule{.15em}{.05em}{.05em}
& \\
\end{tabular} 


}


\caption{Reconstruction results for FOMM \cite{Siarohin_2019_NeurIPS} (re-trained), Articulated Animation (AA) \cite{Siarohin_2021_CVPR} (re-trained), face-vid2vid (f-v2v) \cite{Wang_2021_CVPR} (reported) and our approach on face datasets (\texttt{VoxCeleb}, \texttt{DFDC}, \texttt{Nemo}) and body datasets (\texttt{Fashion}, \texttt{AIST}, \texttt{Tai-Chi-HD}). Results are reported in mean format with best ones bolded. The number of reconstruction testing samples are listed in parentheses behind each dataset name. $\downarrow$ ($\uparrow$) denotes that lower (higher) is better. For \texttt{VoxCeleb} and \texttt{DFDC} which including talking heads, we additionally compute face-only errors for \texttt{L1} and \texttt{LPIPS} (listed in parentheses behind corresponding metrics). Our approach consistently achieves the best performance on \textit{all} metrics across \textit{all six} datasets.
}
\label{tab: recon_body}
\end{table}

==> sub/tab/archive/tab_recon_face.tex <==

\begin{table}[!th] 
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{1.0\linewidth}{!}{
%\hspace{-1cm}
\begin{tabular}{cccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

Dataset & Method & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} \\

\specialrule{.15em}{.05em}{.05em}
%\hlineå



\multicolumn{1}{c}{\multirow{4}{*}{\shortstack{\texttt{VoxCeleb}\\(507)}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.047 (0.22) & 0.14 (0.13) & 50.96 & (0.84) 0.75 & 22.74 & 2.29  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.044 (0.22) & 0.13 (0.22) & 50.69 & (0.86) 0.77 & 23.18 & 2.15  \\ 

& \textit{f-v2v} \cite{Wang_2021_CVPR} & 0.042 (N/A) & N/A (N/A) & 69.13 & (0.85) 0.80 & 24.37 & 2.07  \\ 

& \textit{Ours} & {\bf{0.027}} ({\bf{0.22}}) & {\bf{0.071}} ({\bf{0.22}}) & {\bf{25.43}} & ({\bf{0.93}}) {\bf{0.86}} & {\bf{25.20}} & {\bf{1.90}}    \\ 
  
%%%%%%%%%%%
\specialrule{.08em}{.05em}{.05em}
%\hline
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\td{\texttt{DFDC}}\\\td{(200)}}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} &  &  &   &   &   &    \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} &  &  &   &   &   &    \\  

& \textit{Ours} &  &  &   &   &   &    \\ 
  

%%%%%%%%%%%
\specialrule{.08em}{.05em}{.05em}
%\hline
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Nemo}\\(124)}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.0139  & 0.034 & 19.60 & (0.96) 0.95 & 32.90 & 1.17   \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.0169 & 0.041 & 30.09 & (0.95) 0.93 & 30.55 & 1.32 \\  

& \textit{Ours} & {\bf{0.0061}} & {\bf{0.013}} & {\bf{10.35}} & {\bf{0.99}} ({\bf{0.98}}) & {\bf{39.40}} & {\bf{0.87}}   \\ 

\specialrule{.15em}{.05em}{.05em}
& \\
\end{tabular} 


}

\caption{Reconstruction results for FOMM \cite{Siarohin_2019_NeurIPS} (re-trained), Articulated Animation (AA) \cite{Siarohin_2021_CVPR} (re-trained), face-vid2vid (f-v2v) \cite{Wang_2021_CVPR} (reported) and our approach on face datasets (\texttt{VoxCeleb}, \texttt{DFDC}, \texttt{Nemo}) and body datasets (\texttt{Fashion}, \texttt{AIST}, \texttt{Tai-Chi-HD}). Results are reported in mean format with best ones bolded. The number of reconstruction testing samples are listed in parentheses behind each dataset name. $\downarrow$ ($\uparrow$) denotes that lower (higher) is better. For \texttt{VoxCeleb} and \texttt{DFDC} which including talking heads, we additionally compute face-only errors for \texttt{L1} and \texttt{LPIPS} (listed in parentheses behind corresponding metrics). Our approach consistently achieves the best performance on \textit{all} metrics across \textit{all six} datasets.
}
\label{tab: recon_face}
\end{table}

==> sub/tab/archive/tab_recon_face_body.tex <==

\begin{table*}[!th] 
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{1.0\linewidth}{!}{
%\hspace{-1cm}
\begin{tabular}{ccccccccccccccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

 \multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{6}{c}{\texttt{VoxCeleb} (507)} & \multicolumn{6}{c}{\td{\texttt{DFDC} (200)}} & \multicolumn{6}{c}{\texttt{Nemo} (124)} \\
%\cline{2-9}
\cmidrule(lr){2-7}
\cmidrule(lr){8-13}
\cmidrule(lr){14-19}

& \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} 
& \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} 
& \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} \\

\specialrule{.15em}{.05em}{.05em}
%\hline

\textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.047 (0.22) & 0.14 (0.13) & 50.96 & (0.84) 0.75 & 22.74 & 2.29 &  &   &   &   &   &   & 0.0139  & 0.034 & 19.60 & (0.96) 0.95 & 32.90 & 1.17 \\ 

\textit{AA} \cite{Siarohin_2021_CVPR} & 0.044 (0.22) & 0.13 (0.22) & 50.69 & (0.86) 0.77 & 23.18 & 2.15 &  &  &  &  &  &  & 0.0169 & 0.041 & 30.09 & (0.95) 0.93 & 30.55 & 1.32 \\ 

\textit{f-v2v} \cite{Wang_2021_CVPR} & 0.042 (N/A) & N/A (N/A) & 69.13 & (0.85) 0.80 & 24.37 & 2.07 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A \\ 

\textit{Ours} & {\bf{0.027}} ({\bf{0.22}}) & {\bf{0.071}} ({\bf{0.22}}) & {\bf{25.43}} & ({\bf{0.93}}) {\bf{0.86}} & {\bf{25.20}} & {\bf{1.90}} &   &   &   &   &   &   & {\bf{0.0061}} & {\bf{0.013}} & {\bf{10.35}} & {\bf{0.99}} ({\bf{0.98}}) & {\bf{39.40}} & {\bf{0.87}}   \\ 
  
\specialrule{.08em}{.05em}{.05em}
\specialrule{.08em}{.05em}{.05em}



 \multicolumn{1}{c}{\multirow{2}{*}{Method}}  & \multicolumn{6}{c}{\texttt{Fashion} (100)} & \multicolumn{6}{c}{\td{\texttt{AIST} (200)}} & \multicolumn{6}{c}{\texttt{Tai-Chi-HD} (87)} \\
%\cline{2-9}
\cmidrule(lr){2-7}
\cmidrule(lr){8-13}
\cmidrule(lr){14-19}

& \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} 
& \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} 
& \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} \\


\specialrule{.15em}{.05em}{.05em}
%\hline

\textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.013 & 0.033 & 30.73 & (0.96) 0.93 & 27.06 & 1.09 &  &   &   &   &   &   & 0.057 & 0.24 & 123.78 & (0.69) 0.64 & 20.45 & 9.69 \\ 

\textit{AA} \cite{Siarohin_2021_CVPR} & 0.015 & 0.040 & 37.99 & (0.95) 0.92 & 25.88 & 1.54 &  &  &  &  &  &  & 0.059 & 0.21 & 109.56 & (0.70) 0.57 & 20.31 & 7.30 \\ 

\textit{Ours} & {\bf{0.010}} & {\bf{0.030}} & {\bf{22.25}} & ({\bf{0.95}}) {\bf{0.97}} & {\bf{26.95}} & {\bf{1.00}} &   &   &   &   &   &   & {\bf{0.035}} & {\bf{0.15}} & {\bf{76.41}} & ({\bf{0.83}}) {\bf{0.78}} & {\bf{23.08}} & {\bf{6.36}} \\ 
  
\specialrule{.15em}{.05em}{.05em}
\end{tabular} 


}

\caption{Reconstruction results for FOMM \cite{Siarohin_2019_NeurIPS} (re-trained), Articulated Animation (AA) \cite{Siarohin_2021_CVPR} (re-trained), face-vid2vid (f-v2v) \cite{Wang_2021_CVPR} (reported) and our approach on face datasets (\texttt{VoxCeleb}, \texttt{DFDC}, \texttt{Nemo}) and body datasets (\texttt{Fashion}, \texttt{AIST}, \texttt{Tai-Chi-HD}). Results are reported in mean format with best ones bolded. The number of reconstruction testing samples are listed in parentheses behind each dataset name. $\downarrow$ ($\uparrow$) denotes that lower (higher) is better. For \texttt{VoxCeleb} and \texttt{DFDC} which including talking heads, we additionally compute face-only errors for \texttt{L1} and \texttt{LPIPS} (listed in parentheses behind corresponding metrics). Our approach consistently achieves the best performance on \textit{all} metrics across \textit{all six} datasets.
}
\label{tab: recon_face_body}
\end{table*}

==> sub/tab/tab_ablations_vox.tex <==

\begin{table}[!th] 
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{1.0\linewidth}{!}{
%\hspace{-1cm}
\begin{tabular}{ccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline
 
 

 \multicolumn{1}{c}{\multirow{1}{*}{\textbf{\textit{Model}}}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}}  \\

\specialrule{.08em}{.05em}{.05em}
%\hlineå



\textit{Full} & {\bf{0.027}} & {\bf{0.070}}  & {\bf{25.43}} & ({\bf{0.93}}) {\bf{0.86}} & {\bf{26.20}} & {\bf{1.18}}  \\ 

\textit{w/o Conf.} & {{0.029}}   & {{0.076}}  & {{29.93}} & ({{0.92}}) {{0.84}} & {{26.20}} & {{1.20}}  \\

\textit{w/o Mot. Evol.} & 0.033   & 0.089   & 32.42 & (0.90) 0.83 & 25.27 & 2.04  \\ 

\textit{w/o App.  Assist.} & 0.031   & 0.085   & 32.12 & (0.91) 0.84 & 25.96 & 1.94    \\ 

\textit{w/o Mult. Fus.} & 0.043   & 0.133   & 42.92 & (0.86) 0.78 & 23.99 & 2.30    \\ 


\specialrule{.15em}{.05em}{.05em} 
\end{tabular} 


}

\caption{Ablations results of the proposed framework on \texttt{VoxCeleb} dataset (507 testing samples for reconstruction), with mean results reported and best ones bolded. $\downarrow$ ($\uparrow$) denotes that lower (higher) is better.
}

\label{tab: ablations}
\end{table}

==> sub/tab/tab_all_eight.tex <==

\begin{table*}[h] 
\centering
\renewcommand{\arraystretch}{1.25}
\resizebox{1.0\linewidth}{!}{
%\hspace{-1cm}
 
\begin{tabular}{cccccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

\multicolumn{1}{c}{\multirow{2}{*}{\textbf{\textit{Dataset}}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\textit{Method}}}} & \multicolumn{6}{c}{\textbf{\textit{Video Reconstruction}}} & \multicolumn{2}{c}{\textbf{\textit{Image Animation}}} \\

\cmidrule(lr){3-8}
\cmidrule(lr){9-10}

&  & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{MS-/SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} & {\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{CSIM} ($\uparrow$)}} \\

\specialrule{.15em}{.05em}{.05em}
%\hline

\multicolumn{1}{c}{\multirow{4}{*}{\shortstack{\texttt{VoxCeleb}\\(507)}}} &  \texttt{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.047 (0.040) & 0.14 (0.11)  & 50.96 (43.28) & 0.84/0.75 (0.87/0.78) & 22.74 (23.77) & 2.29 (1.36) & 62.88 (52.10) & 0.78 (0.81) \\ 

& \texttt{AA} \cite{Siarohin_2021_CVPR} & 0.044 (0.034)  & 0.13 (0.18) & 50.69 (44.02) & 0.86/0.77 (0.90/0.82) & 23.18 (24.61) & 2.15 (1.26) & 86.03 (79.59) & 0.75 (0.75) \\ 

& \texttt{f-v2v} \cite{Wang_2021_CVPR} & 0.042 & N/A  & 69.13 & 0.85/0.80 & 24.37 & 2.07 & 55.64 & 0.75  \\ 

& \texttt{SLIDE} & {\bf{0.027}}   & {\bf{0.070}}  & {\bf{25.43}} & {\bf{0.93}}/{\bf{0.86}} & {\bf{26.20}} & {\bf{1.18}} & {\bf{47.21}} & {\bf{0.90}}  \\ 
  
%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{DFDC}\\(1807)}}} &  \texttt{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.034 (0.029) & 0.140 (0.119) & 61.59 (51.59) & 0.86/0.80 (0.89/0.82) & 25.65 (26.72)  &  2.81 (2.42) & 84.18 (78.76) & 0.81 (0.85) \\ 

& \texttt{AA} \cite{Siarohin_2021_CVPR} & 0.039 (0.035) & 0.156 (0.140) & 89.88 (83.79)  & 0.86/0.79 (0.89/0.80)  & 23.64 (24.21) & 2.52 (2.43) & 172.35 (156.32) & 0.73 (0.74) \\  

& \texttt{SLIDE} & {\bf{0.018}}  & {\bf{0.0061}} & {\bf{33.22}} & {\bf{0.95}}/{\bf{0.91}} & {\bf{27.99}} & {\bf{1.28}}  & {\bf{64.89}} & {\bf{0.92}}   \\ 
  

%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{UvA-Nemo}\\(124)}}} &  \texttt{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.0139 (0.0120) & 0.034 (0.027) & 19.60 (18.03) & 0.96/0.95 (0.97/0.95) & 32.90 (33.91) & 1.17 (1.12) & 27.46 (23.80) & 0.93 (0.94) \\ 

& \texttt{AA} \cite{Siarohin_2021_CVPR} & 0.0169 (0.0151) & 0.041 (0.037) & 30.09 (40.31) & 0.95/0.93 (0.96/0.94) & 30.55 (31.00) & 1.32 (1.24) & 72.11 (67.65) & 0.83 (0.83) \\  

& \texttt{SLIDE} & {\bf{0.0061}} & {\bf{0.013}} & {\bf{10.35}} & {\bf{0.99}}/{\bf{0.98}} & {\bf{39.40}} & {\bf{0.87}} & {\bf{23.46}} & {\bf{0.98}} \\ 


%%%%%%%%%%%
\specialrule{.08em}{.05em}{.05em}
\specialrule{.08em}{.05em}{.05em}
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{AIST}\\(493)}}} &  \texttt{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.015 (0.013)  & 0.056 (0.048) & 63.17 (49.33) & 0.94/0.94 (0.95/0.94) & 26.27 (26.92) & 6.69 (5.47)  & 114.57 (109.81) & 0.99 (0.99)  \\ 

& \texttt{AA} \cite{Siarohin_2021_CVPR} & 0.029 (0.028) & 0.239 (0.234) & 99.95 (91.93) & 0.94/0.91 (0.95/0.92) & 20.40 (20.54) & 5.67 (5.09) & 198.43 (182.63) & 0.98 (0.99) \\  

& \texttt{SLIDE} & {\bf{0.011}} & {\bf{0.043}} & {\bf{37.71}} & {\bf{0.96}}/{\bf{0.95}} & {\bf{26.97}} & {\bf{3.66}}  & {\bf{105.20}} & {\bf{0.99}}    \\ 
  
%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Tai-Chi-HD}\\(87)}}} &  \texttt{FOMM} \cite{Siarohin_2019_NeurIPS}  & 0.057 (0.046) & 0.24 (0.18) & 123.78 (95.95) & 0.69/0.64 (0.77/0.72) & 20.45 (21.73) & 9.69 (7.87) & 148.86 (134.46) & 0.99 (0.99) \\ 

& \texttt{AA} \cite{Siarohin_2021_CVPR} & 0.059 (0.053) & 0.21 (0.17) & 109.56 (86.57) & 0.70/0.57 (0.76/0.63) & 20.31 (21.19) & 7.30 (6.67) & 159.54 (147.73) & 0.99 (0.99) \\  

& \texttt{SLIDE}  & {\bf{0.035}} & {\bf{0.15}} & {\bf{76.41}} & {\bf{0.83}}/{\bf{0.78}} & {\bf{23.08}} & {\bf{6.36}} & {\bf{123.10}} & {\bf{0.99}} \\ 
  
%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Fashion}\\(100)}}} &  \texttt{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.013 (0.013) & 0.033 (0.033) & 30.73 (30.18) & 0.96/0.93 (0.95/0.93) & 27.06 (26.12) & 1.09 (1.08) & 41.10 (39.52) & 0.99 (0.99) \\ 

& \texttt{AA} \cite{Siarohin_2021_CVPR} & 0.015 (0.014) & 0.040 (0.039) & 37.99 (36.10) & 0.95/0.92 (0.96/0.92) & 25.88 (25.98) & 1.54 (1.50) & 78.01 (70.76) & 0.99 (0.99) \\  

& \texttt{SLIDE} & {\bf{0.010}} & {\bf{0.030}} & {\bf{22.25}} & {\bf{0.97}}/{\bf{0.95}} & {\bf{26.95}} & {\bf{1.00}} & {\bf{32.64}} & {\bf{0.99}} \\ 


%%%%%%%%%%%
\specialrule{.08em}{.05em}{.05em}
\specialrule{.08em}{.05em}{.05em}
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Bair}\\(128)}}} & \texttt{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.030 (0.024) & 0.067 (0.047) & 107.70 (45.41) & 0.91/0.88 (0.94/0.91) & 23.64 (25.35) & N/A & 107.70 (114.54) & N/A \\ 

& \texttt{AA} \cite{Siarohin_2021_CVPR} & 0.052 (0.048) & 0.137 (0.121) & 217.87 (77.14) & 0.87/0.76 (0.90/0.77) & 19.75 (19.75)  & N/A & 217.87 (201.78) & N/A\\ 

& \texttt{SLIDE} & {\bf{0.018}} & {\bf{0.027}} & {\bf{34.44}} & {\bf{(0.97) 0.94}} & {\bf{27.75}} & N/A & {\bf{96.91}} & N/A \\ 


%%%%%%%%%%%
\specialrule{.08em}{.05em}{.05em}
\specialrule{.08em}{.05em}{.05em}
%%%%%%%%%%%
 
\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{MGif}\\(100)}}} & \texttt{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.033 (0.031) & 0.112 (0.106) & 154.88 (146.46) & 0.87/0.84 (0.87/0.84) & 19.56 (19.79) & N/A & 196.94 (183.68) & N/A \\ 

& \texttt{AA} \cite{Siarohin_2021_CVPR} & 0.026 (0.026) & 0.092 (0.089) & 136.84 (131.89) & 0.90/0.85 (0.90/0.86) & 20.22 (20.35) & N/A & 331.72 (315.71) & N/A \\ 

& \texttt{SLIDE} & {\bf{0.021}} & {\bf{0.072}} & {\bf{117.74}} & {\bf{(0.92) 0.90}} & {\bf{21.34}} & N/A & {\bf{180.30}} & N/A \\ 

\specialrule{.15em}{.05em}{.05em}
 
\end{tabular} 
}

%\vspace{-0.2cm}

\caption{Comparing \texttt{FOMM} \cite{Siarohin_2019_NeurIPS}, Articulated Animation (\texttt{AA}) \cite{Siarohin_2021_CVPR}, \texttt{face-vid2vid} (f-v2v) \cite{Wang_2021_CVPR} (reported) and \texttt{SLIDE} on human face datasets (\texttt{VoxCeleb}, \texttt{DFDC}, \texttt{UvA-Nemo}), human body datasets (\texttt{AIST}, \texttt{Tai-Chi-HD, \texttt{Fashion}}), robot dataset (\texttt{Bair}) and cartoon animal dataset (\texttt{MGif}). The number of reconstruction testing samples are listed in parentheses below each dataset name. For animation tests, 200 source-driving object pairs are randomly generated for each dataset. Results are reported in mean format with best ones bolded. $\downarrow$ ($\uparrow$) denotes that lower (higher) is better. For one-shot baseline models, we additionally list, in the parentheses, the best scores computed from the same reference images used by \texttt{SLIDE}. Clearly, \texttt{SLIDE} consistently achieves the best performance on \textit{all} metrics across \textit{all} eight datasets.
}
\label{tab: all}
\end{table*}



==> sub/tab/tab_anim_all.tex <==

\begin{table*}[!th] 
\centering
\renewcommand{\arraystretch}{1.}

\resizebox{1.0\linewidth}{!}{
\begin{tabular}{ccccccccccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

 \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\textit{Method}}}}  & \multicolumn{2}{c}{\texttt{VoxCeleb}} & \multicolumn{2}{c}{\td{\texttt{DFDC}}} & \multicolumn{2}{c}{\texttt{Nemo}}
 & \multicolumn{2}{c}{\texttt{Fashion}} & \multicolumn{2}{c}{\td{\texttt{AIST}}} & \multicolumn{2}{c}{\texttt{Tai-Chi-HD}}
 & \multicolumn{1}{c}{\texttt{Bair}} & \multicolumn{1}{c}{\td{\texttt{MGif}}}  \\
%\cline{2-9}
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
\cmidrule(lr){10-11}
\cmidrule(lr){12-13}
\cmidrule(lr){14-14} 
\cmidrule(lr){15-15} 

& {\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{CSIM} ($\uparrow$)}}
& {\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{CSIM} ($\uparrow$)}}
& {\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{CSIM} ($\uparrow$)}}
& {\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{CSIM} ($\uparrow$)}}
& {\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{CSIM} ($\uparrow$)}}
& {\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{CSIM} ($\uparrow$)}}
& {\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} \\

\specialrule{.08em}{.05em}{.05em}

\textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 62.88 & 0.78 & & & 27.46 & 0.99 & 41.10 & 0.99 & & & 148.86 & 0.99 & 107.70 & 196.94 \\ 

\textit{AA} \cite{Siarohin_2021_CVPR} & 86.03 & 0.75 & & & 72.11 & 0.99 & 78.01 & 0.99 & & & 159.54 & 0.99 & 217.87 & 331.72 \\ 

\textit{f-v2v} \cite{Wang_2021_CVPR} & 55.64 & 0.75 & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A \\ 

\textit{Ours} & {\bf{47.41}} & {\bf{0.83}} &  &  & {\bf{23.46}} & {\bf{0.99}} & {\bf{32.64}} & {\bf{0.99}} & & & {\bf{134.46}} & {\bf{0.99}} & {\bf{96.91}} & {\bf{180.30}} \\ 
  
\specialrule{.15em}{.05em}{.05em}
\end{tabular} 


}

\caption{Animation results for FOMM \cite{Siarohin_2019_NeurIPS} (re-trained), Articulated Animation (AA) \cite{Siarohin_2021_CVPR} (re-trained), face-vid2vid (f-v2v) \cite{Wang_2021_CVPR} (reported) and our approach on \td{eight} datasets. Results are reported in mean format with best ones bolded. The number of randomly assigned animation pairs are 200 for all datasets. $\downarrow$ ($\uparrow$) denotes that lower (higher) is better. Our approach consistently achieves the best performance on \textit{all} metrics across \textit{all} datasets.
}
\label{tab: anim_all}
\end{table*}

==> sub/tab/tab_gen_num_refs.tex <==
  \begin{minipage}{\textwidth} 
  \hspace{-0.6cm}
  \begin{minipage}[b]{0.49\textwidth}
    \centering 
    \renewcommand{\arraystretch}{1.2}
    \resizebox{1.0\linewidth}{!}{
    %\hspace{-1cm}
    \begin{tabular}{ccccccccc}
    \specialrule{.15em}{.05em}{.05em}
    %\hline
    
    \multicolumn{1}{l}{\multirow{2}{*}{{$\mathbf{N}$}}} & \multicolumn{6}{c}{\multirow{1}{*}{\textbf{\textit{\hypertarget{tab: num_refs_all}{Reconstruction}}}}} & \multicolumn{2}{c}{\multirow{1}{*}{\textbf{\textit{Animation}}}} \\
    
    \cmidrule(lr){2-7}
    \cmidrule(lr){8-9}
    
     & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{MS-/SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{CSIM} ($\uparrow$)}}\\
    
    \specialrule{.08em}{.05em}{.05em}
    %\hline
    
    
    \textit{1} & 0.024   & 0.088   & 42.20 & 0.90/0.87 & 27.23 & 1.33 & 68.78 & 0.89 \\ 
    
    \textit{2} & 0.021   & 0.070   & 35.34 & 0.93/0.89 & 27.35 & 1.34 & 67.58 & 0.90 \\ 
    
    \textit{3} & 0.018 & 0.0061  & 33.22 & 0.95/0.91 & 27.99 & 1.28 & 64.89 & 0.92 \\ 
    
    \textit{4} & 0.017   & 0.058   & 31.89 & 0.95/0.92 & 28.56 & 1.24 & 64.82 & 0.92 \\ 
    
    \textit{5} & 0.017   & 0.051   & 30.69 & 0.96/0.92 & 28.83 & 1.21 & 65.15 & 0.92 \\ 
    
    \textit{6} &   0.016  &  0.050   &  31.17 &  0.96/0.92  &  29.04 & 1.19  & 64.86 & 0.92   \\ 
    
    
    \specialrule{.15em}{.05em}{.05em}
     %\multicolumn{8}{l}{\multirow{1}{*}{\small{(*: equals to the full model used in this paper)}}} 
    \end{tabular}  
    }
    \captionof{table}{Ablation results for different additional view numbers ($N$), tested on \texttt{DFDC} (1807 testing samples for reconstruction, 200 testing pairs for animation), with mean results reported and best ones bolded. $\downarrow$ ($\uparrow$) denotes that lower (higher) is better.}
    \end{minipage}
  ~
  \begin{minipage}[b]{0.49\textwidth} 
\centering
\renewcommand{\arraystretch}{1.28}
\resizebox{1.0\linewidth}{!}{
%\hspace{-1cm}
%(a)
\begin{tabular}{cccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

{\textbf{\textit{\hypertarget{tab: gen_all}{Dataset}}}} & {\textbf{\textit{Method}}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{MS-/SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} \\

\specialrule{.08em}{.05em}{.05em}
%\hlineå

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Nemo}\\(124)}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.0191  & 0.047 & 37.57 & 0.94/0.91 & 29.93 & 1.36    \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.0170 & 0.045 & 33.95 & 0.95/0.92 & 30.38 & 1.24 \\  

& \textit{Ours (0)}& 0.0159 & 0.044 & 36.47 & 0.96/0.93 & 31.08 & 1.24 \\  

& \textit{Ours} & {\bf{0.0086}} & {\bf{0.023}} & {\bf{29.45}} & {\bf{0.99}}/{\bf{0.97}} & {\bf{36.80}} & {\bf{0.98}}   \\ 

%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%
 
\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{MGif}\\(100)}}} & \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.086 & 0.256 & 222.99 & 0.76/0.63 & 15.38 & N/A  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.102 & 0.345 & 269.44 & 0.57/0.73 & 14.82 & N/A \\ 

& \textit{Ours} & {\bf{0.045}} & {\bf{0.176}} & {\bf{158.96}} & {\bf{0.81/0.86}} & {\bf{18.70}} & N/A \\ 
 
\specialrule{.15em}{.05em}{.05em} 
\end{tabular} 
}
  \captionof{table}{Model generality results for FOMM \cite{Siarohin_2019_NeurIPS}, Articulated Animation (AA) \cite{Siarohin_2021_CVPR} and our approach. Results computed based on models trained on \texttt{VoxCeleb} dataset, while tested on \texttt{Nemo} (face) and \texttt{MGif} (cartoons) datasets.}
  \end{minipage}
  \end{minipage}

==> sub/tab/tab_num_refs.tex <==

\begin{table}[!th] 
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{1.0\linewidth}{!}{
%\hspace{-1cm}
\begin{tabular}{ccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

%\cmidrule(lr){2-7} 

\multicolumn{1}{l}{\multirow{1}{*}{{$\mathbf{N}$}}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} \\

\specialrule{.08em}{.05em}{.05em}
%\hlineå


\textit{1} & 0.033   & 0.089   & 32.42 & 0.90/0.83 & 25.27 & 2.04 \\ 

\textit{2} & 0.033   & 0.089   & 32.42 & 0.90/0.83 & 25.27 & 2.04 \\ 

\textit{3*} & 0.027 & 0.071  & 25.43 & 0.90/0.83 & 26.20 & 1.90 \\ 

\textit{4} & 0.033   & 0.089   & 32.42 & 0.90/0.83 & 25.27 & 2.04  \\ 

\textit{5} & 0.031   & 0.085   & 32.12 & 0.90/0.83 & 25.96 & 1.94  \\ 

\textit{6} & 0.043   & 0.133   & 42.92 & 0.90/0.83 & 23.99 & 2.30  \\ 


\specialrule{.15em}{.05em}{.05em}
 \multicolumn{7}{l}{\multirow{1}{*}{\small{(*: equals to the full model used in this paper)}}}

\end{tabular} 

}

\caption{Reconstruction results for testing with different number ($N$) of reference images, on \texttt{VoxCeleb} dataset (over 507 testing samples), with mean results reported and best ones bolded. $\downarrow$ ($\uparrow$) denotes that lower (higher) is better. 
}

\label{tab: num_refs}
\end{table}

==> sub/tab/tab_num_refs_all_vox.tex <==

\begin{table}[!th] 
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{1.0\linewidth}{!}{
%\hspace{-1cm}
\begin{tabular}{ccccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

\multicolumn{1}{l}{\multirow{2}{*}{{$\mathbf{N}$}}} & \multicolumn{6}{c}{\multirow{1}{*}{\textbf{\textit{Reconstruction}}}} & \multicolumn{2}{c}{\multirow{1}{*}{\textbf{\textit{Animation}}}} \\

\cmidrule(lr){2-7}
\cmidrule(lr){8-9}

 & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{MS-/SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{CSIM} ($\uparrow$)}}\\

\specialrule{.08em}{.05em}{.05em}
%\hline


\textit{1} & 0.030   & 0.083   & 28.07 & 0.90/0.83 & 25.39 & 1.25 & 51.65 & 0.88 \\ 

\textit{2} & 0.030   & 0.083   & 27.27 & 0.91/0.84 & 25.46 & 1.23 & 48.16 & 0.89  \\ 

\textit{3*} & 0.027 & 0.070  & 25.43 & 0.93/0.86 & 26.20 & 1.18 & 47.21 & 0.90 \\ 

\textit{4} & 0.027   & 0.069   & 27.13 & 0.93/0.86 & 26.46 & 1.16 & 47.75 & 0.89  \\ 

\textit{5} & 0.026   & 0.075   & 26.29 & 0.94/0.86 & 27.02 & 1.14 & 49.76 & 0.88  \\ 

\textit{6} & 0.025   & 0.063   & 25.51 & 0.94/0.87 & 27.18 & 1.13 & 49.33 & 0.89  \\ 


\specialrule{.15em}{.05em}{.05em}
 \multicolumn{8}{l}{\multirow{1}{*}{\small{(*: equals to the full model used in this paper)}}}

\end{tabular} 

}

\caption{Reconstruction \& animation results for different choices of additional source view numbers ($N$), tested on \texttt{VoxCeleb} dataset (507 testing samples for reconstruction task, 200 testing pairs for animation), with mean results reported and best ones bolded. $\downarrow$ ($\uparrow$) denotes that lower (higher) is better. 
}

\label{tab: num_refs_all}
\end{table}

==> sub/tab/tab_num_refs_vox.tex <==

\begin{table}[!th] 
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{1.0\linewidth}{!}{
%\hspace{-1cm}
\begin{tabular}{ccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

%\cmidrule(lr){2-7} 

\multicolumn{1}{l}{\multirow{1}{*}{{$\mathbf{N}$}}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} \\

\specialrule{.08em}{.05em}{.05em}
%\hlineå


\textit{1} & 0.033   & 0.089   & 32.42 & 0.90/0.83 & 25.27 & 2.04 \\ 

\textit{2} & 0.033   & 0.089   & 32.42 & 0.90/0.83 & 25.27 & 2.04 \\ 

\textit{3*} & 0.027 & 0.071  & 25.43 & 0.90/0.83 & 26.20 & 1.90 \\ 

\textit{4} & 0.033   & 0.089   & 32.42 & 0.90/0.83 & 25.27 & 2.04  \\ 

\textit{5} & 0.031   & 0.085   & 32.12 & 0.90/0.83 & 25.96 & 1.94  \\ 

\textit{6} & 0.043   & 0.133   & 42.92 & 0.90/0.83 & 23.99 & 2.30  \\ 


\specialrule{.15em}{.05em}{.05em}
 \multicolumn{7}{l}{\multirow{1}{*}{\small{(*: equals to the full model used in this paper)}}}

\end{tabular} 

}

\caption{Reconstruction results for testing with different number ($N$) of reference images, on \texttt{VoxCeleb} dataset (over 507 testing samples), with mean results reported and best ones bolded. $\downarrow$ ($\uparrow$) denotes that lower (higher) is better. 
}

\label{tab: num_refs}
\end{table}

==> sub/tab/tab_recon_all.tex <==

\begin{table}[!th] 
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{1.0\linewidth}{!}{
%\hspace{-1cm}
(a)
\begin{tabular}{cccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

{\textbf{\textit{Dataset}}} & {\textbf{\textit{Method}}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} \\

\specialrule{.08em}{.05em}{.05em}
%\hlineå



\multicolumn{1}{c}{\multirow{4}{*}{\shortstack{\texttt{VoxCeleb}\\(507)}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.047  & 0.14  & 50.96 & (0.84) 0.75 & 22.74 & 2.29  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.044  & 0.13  & 50.69 & (0.86) 0.77 & 23.18 & 2.15  \\ 

& \textit{f-v2v} \cite{Wang_2021_CVPR} & 0.042 & N/A  & 69.13 & (0.85) 0.80 & 24.37 & 2.07  \\ 

& \textit{Ours} & {\bf{0.027}}   & {\bf{0.071}}  & {\bf{25.43}} & ({\bf{0.93}}) {\bf{0.86}} & {\bf{26.20}} & {\bf{1.90}}    \\ 
  
%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\td{\texttt{DFDC}}\\\td{(200)}}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.029  & 0.106 & 61.06  &  (0.88) 0.84 & 25.58  &  1.58  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.034 & 0.129 & 83.04  & (0.87) 0.80  & 23.29  & 1.48   \\  

& \textit{Ours} & {\bf{0.021}}   & {\bf{0.075}}  & {\bf{51.14}} & ({\bf{0.93}}) {\bf{0.88}} & {\bf{28.45}} & {\bf{1.46}}    \\ 
  

%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Nemo}\\(124)}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.0139  & 0.034 & 19.60 & (0.96) 0.95 & 32.90 & 1.17   \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.0169 & 0.041 & 30.09 & (0.95) 0.93 & 30.55 & 1.32 \\  

& \textit{Ours} & {\bf{0.0061}} & {\bf{0.013}} & {\bf{10.35}} & ({\bf{0.99}}) {\bf{0.98}} & {\bf{39.40}} & {\bf{0.87}}   \\ 

\specialrule{.15em}{.05em}{.05em} 
\end{tabular} 


}



\resizebox{1.0\linewidth}{!}{
(b)
\begin{tabular}{cccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

{\textbf{\textit{Dataset}}} & {\textbf{\textit{Method}}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} \\

\specialrule{.08em}{.05em}{.05em}
%\hlineå



\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Fashion}\\(100)}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.013 & 0.033 & 30.73 & (0.96) 0.93 & 27.06 & 1.09  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.015 & 0.040 & 37.99 & (0.95) 0.92 & 25.88 & 1.54  \\  

& \textit{Ours} & {\bf{0.010}} & {\bf{0.030}} & {\bf{22.25}} & ({\bf{0.97}}) {\bf{0.95}} & {\bf{26.95}} & {\bf{1.00}}    \\ 
  
%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%


\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\td{\texttt{AIST}}\\ \td{(200)}}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.018  & 0.152 & 55.98 & (0.94) 0.93 & 23.81 & 5.04 \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.028 & 0.259 & 105.23  & (0.94) 0.92 & 20.30 & 5.33 \\  

& \textit{Ours} & {\bf{0.015}} & {\bf{0.105}} & {\bf{47.89}} & ({\bf{0.95}}) {\bf{0.94}} & {\bf{24.20}} & {\bf{4.86}}    \\ 
  
%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Tai-Chi-HD}\\(87)}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS}  & 0.057 & 0.24 & 123.78 & (0.69) 0.64 & 20.45 & 9.69 \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.059 & 0.21 & 109.56 & (0.70) 0.57 & 20.31 & 7.30   \\  

& \textit{Ours}  & {\bf{0.035}} & {\bf{0.15}} & {\bf{76.41}} & ({\bf{0.83}}) {\bf{0.78}} & {\bf{23.08}} & {\bf{6.36}}  \\ 


\specialrule{.15em}{.05em}{.05em} 
\end{tabular} 


}


\resizebox{1.0\linewidth}{!}{
(c)
\begin{tabular}{ccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

 
%\cmidrule(lr){2-6}

{\textbf{\textit{Dataset}}} & {\textbf{\textit{Method}}} & {\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & {\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & {\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & {\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & {\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}}  \\

\specialrule{.08em}{.05em}{.05em}
%\hline

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Bair}\\(128)}}} & \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.030 & 0.067 & 107.70 & (0.91) 0.88 & 23.64  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.052 & 0.137 & 217.87 & (0.87) 0.76 & 19.75  \\ 

& \textit{Ours} & {\bf{0.018}} & {\bf{0.027}} & {\bf{34.44}} & {\bf{(0.97) 0.94}} & {\bf{27.75}}  \\ 


%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%
 
\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{MGif}\\(100)}}} & \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.033 & 0.112 & 154.88 & (0.87) 0.84 & 19.56  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.026 & 0.092 & 136.84 & (0.90) 0.85 & 20.22 \\ 

& \textit{Ours} & {\bf{0.021}} & {\bf{0.072}} & {\bf{117.74}} & {\bf{(0.92) 0.90}} & {\bf{21.34}} \\ 
  
\specialrule{.15em}{.05em}{.05em}
 
\end{tabular} 
}


\caption{Reconstruction results for FOMM \cite{Siarohin_2019_NeurIPS} (re-trained), Articulated Animation (AA) \cite{Siarohin_2021_CVPR} (re-trained), face-vid2vid (f-v2v) \cite{Wang_2021_CVPR} (reported) and our approach on (a) face datasets (\texttt{VoxCeleb}, \texttt{DFDC}, \texttt{Nemo}), (b) body datasets (\texttt{Fashion}, \texttt{AIST}, \texttt{Tai-Chi-HD}) and (c) robot (\texttt{Bair}) \& cartoon animals (\texttt{MGif}) datasets. Results are reported in mean format with best ones bolded. The number of reconstruction testing samples are listed in parentheses below each dataset name. $\downarrow$ ($\uparrow$) denotes that lower (higher) is better.  Our approach consistently achieves the best performance on \textit{all} metrics across \textit{all} eight datasets.
}
\label{tab: recon_all}
\end{table}

==> sub/tab/tab_recon_all_3_.tex <==

\begin{table}[!th] 
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{1.0\linewidth}{!}{
%\hspace{-1cm}
(a)
\begin{tabular}{cccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

{\textbf{\textit{Dataset}}} & {\textbf{\textit{Method}}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} \\

\specialrule{.08em}{.05em}{.05em}
%\hlineå



\multicolumn{1}{c}{\multirow{4}{*}{\shortstack{\texttt{\td{VoxCeleb}}\\\td{(507)}}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} &   &   &   &  &   &    \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} &   &   &   &  &   &    \\  

& \textit{Ours} & {\bf{0.027}}   & {\bf{0.071}}  & {\bf{25.43}} & ({\bf{0.93}}) {\bf{0.86}} & {\bf{26.20}} & {\bf{1.90}}    \\ 
  
%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\td{\texttt{DFDC}}\\\td{(200)}}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.023  & 0.084 & 54.67  &  (0.92) 0.87 & 28.21  &  1.66  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.032 & 0.112 & 69.97  & (0.90) 0.82  & 24.11  & 1.60   \\  

& \textit{Ours} & {\bf{0.021}}   & {\bf{0.075}}  & {\bf{51.14}} & ({\bf{0.93}}) {\bf{0.88}} & {\bf{28.45}} & {\bf{1.46}}    \\ 
  

%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Nemo}\\(124)}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.0120  & 0.027 & 18.03 & (0.97) 0.95 & 33.91 & 1.12   \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.0151 & 0.037 & 40.31 & (0.96) 0.94 & 31.00 & 1.24 \\  

& \textit{Ours} & {\bf{0.0061}} & {\bf{0.013}} & {\bf{10.35}} & ({\bf{0.99}}) {\bf{0.98}} & {\bf{39.40}} & {\bf{0.87}}   \\ 

\specialrule{.15em}{.05em}{.05em} 
\end{tabular} 


}



\resizebox{1.0\linewidth}{!}{
(b)
\begin{tabular}{cccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

{\textbf{\textit{Dataset}}} & {\textbf{\textit{Method}}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} \\

\specialrule{.08em}{.05em}{.05em}
%\hlineå



\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Fashion}\\(100)}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.013  & 0.033 & 30.18 & (0.95) 0.93 & 26.12 & 1.08 \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.014 & 0.039 & 36.10  & (0.96) 0.92 & 25.98 & 1.50 \\  

& \textit{Ours} & {\bf{0.010}} & {\bf{0.030}} & {\bf{22.25}} & ({\bf{0.97}}) {\bf{0.95}} & {\bf{26.95}} & {\bf{1.00}}    \\ 
  
%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\td{\texttt{AIST}}\\ \td{(200)}}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.020  & 0.126 & 57.39 & (0.94) 0.93 & 23.49 & 5.51 \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.028 & 0.258 & 95.44  & (0.94) 0.93 & 20.31 & 5.60 \\  

& \textit{Ours} & {\bf{0.015}} & {\bf{0.105}} & {\bf{47.89}} & ({\bf{0.95}}) {\bf{0.94}} & {\bf{24.20}} & {\bf{4.86}}    \\ 
  
%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Tai-Chi-HD}\\(87)}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS}  & 0.046 & 0.18 & 95.95 & (0.77) 0.72 & 21.73 & 7.87  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.053 & 0.17 & 86.54 & (0.76) 0.63 & 21.19 & 6.67   \\  

& \textit{Ours}  & {\bf{0.035}} & {\bf{0.15}} & {\bf{76.41}} & ({\bf{0.83}}) {\bf{0.78}} & {\bf{23.08}} & {\bf{6.36}}  \\ 


\specialrule{.15em}{.05em}{.05em} 
\end{tabular} 


}


\resizebox{1.0\linewidth}{!}{
(c)
\begin{tabular}{ccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

 
%\cmidrule(lr){2-6}

{\textbf{\textit{Dataset}}} & {\textbf{\textit{Method}}} & {\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & {\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & {\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & {\multirow{1}{*}{\texttt{(MS-)SSIM} ($\uparrow$)}} & {\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}}  \\

\specialrule{.08em}{.05em}{.05em}
%\hline

\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Bair}\\(128)}}} & \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.024 & 0.047 & 45.41 & (0.94) 0.91 & 25.35  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.048 & 0.121 & 77.14 & (0.90) 0.77 & 19.75  \\ 

& \textit{Ours} & {\bf{0.018}} & {\bf{0.026}} & {\bf{34.44}} & {\bf{(0.97) 0.94}} & {\bf{27.75}}  \\ 


%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%
 
\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{MGif}\\(100)}}} & \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.031 & 0.106 & 146.46 & (0.87) 0.84 & 19.79  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.026 & 0.089 & 131.89 & (0.90) 0.86 & 20.35 \\ 

& \textit{Ours} & {\bf{0.021}} & {\bf{0.072}} & {\bf{117.74}} & {\bf{(0.92) 0.90}} & {\bf{21.34}} \\ 
  
\specialrule{.15em}{.05em}{.05em}
 
\end{tabular} 
}


\caption{Reconstruction results for FOMM \cite{Siarohin_2019_NeurIPS} (re-trained), Articulated Animation (AA) \cite{Siarohin_2021_CVPR} (re-trained), and our approach on (a) face datasets (\texttt{VoxCeleb}, \texttt{DFDC}, \texttt{Nemo}), (b) body datasets (\texttt{Fashion}, \texttt{AIST}, \texttt{Tai-Chi-HD}) and (c) robot (\texttt{Bair}) \& cartoon animals (\texttt{MGif}) datasets. Results are reported in mean format with best ones bolded. The number of reconstruction testing samples are listed in parentheses below each dataset name. $\downarrow$ ($\uparrow$) denotes that lower (higher) is better.  Our approach consistently achieves the best performance on \textit{all} metrics across \textit{all} eight datasets.
}
\label{tab: recon_all(3)}
\end{table}

==> sub/tab/test_wrap_tab.tex <==
\begin{wraptable}{r}{0.7\textwidth}
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{1.0\linewidth}{!}{
%\hspace{-1cm}
%(a)
\begin{tabular}{cccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

{\textbf{\textit{Dataset}}} & {\textbf{\textit{Method}}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{MS-/SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} \\

\specialrule{.08em}{.05em}{.05em}
%\hlineå



\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{Nemo}\\(124)}}} &  \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.0191  & 0.047 & 37.57 & 0.94/0.91 & 29.93 & 1.36    \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.0170 & 0.045 & 33.95 & 0.95/0.92 & 30.38 & 1.24 \\  

& \textit{Ours (0)}& 0.0159 & 0.044 & 36.47 & 0.96/0.93 & 31.08 & 1.24 \\  

& \textit{Ours} & {\bf{0.0086}} & {\bf{0.023}} & {\bf{29.45}} & {\bf{0.99}}/{\bf{0.97}} & {\bf{36.80}} & {\bf{0.98}}   \\ 



%%%%%%%%%%%
%\specialrule{.08em}{.05em}{.05em}
\hline
%%%%%%%%%%%
 
\multicolumn{1}{c}{\multirow{3}{*}{\shortstack{\texttt{MGif}\\(100)}}} & \textit{FOMM} \cite{Siarohin_2019_NeurIPS} & 0.086 & 0.256 & 222.99 & 0.76/0.63 & 15.38 & N/A  \\ 

& \textit{AA} \cite{Siarohin_2021_CVPR} & 0.102 & 0.345 & 269.44 & 0.57/0.73 & 14.82 & N/A \\ 

& \textit{Ours} & {\bf{0.045}} & {\bf{0.176}} & {\bf{158.96}} & {\bf{0.81/0.86}} & {\bf{18.70}} & N/A \\ 
  

\specialrule{.15em}{.05em}{.05em} 
\end{tabular} 
}
%\vspace{-0.5cm}
\caption{Model generality results for FOMM \cite{Siarohin_2019_NeurIPS}, Articulated Animation (AA) \cite{Siarohin_2021_CVPR} and our approach. Results computed based on models trained on \texttt{VoxCeleb} dataset, while tested on \texttt{Nemo} (face) and \texttt{MGif} (cartoons) datasets. 
}
\label{tab: gen_all}
\end{wraptable}

==> sub/tab/test_wrap_tab2.tex <==

\begin{wraptable}{r}{0.5\textwidth}
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{1.0\linewidth}{!}{
%\hspace{-1cm}
\begin{tabular}{ccccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline

\multicolumn{1}{l}{\multirow{2}{*}{{$\mathbf{N}$}}} & \multicolumn{6}{c}{\multirow{1}{*}{\textbf{\textit{Reconstruction}}}} & \multicolumn{2}{c}{\multirow{1}{*}{\textbf{\textit{Animation}}}} \\

\cmidrule(lr){2-7}
\cmidrule(lr){8-9}

 & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{MS-/SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{CSIM} ($\uparrow$)}}\\

\specialrule{.08em}{.05em}{.05em}
%\hline


\textit{1} & 0.024   & 0.088   & 42.20 & 0.90/0.87 & 27.23 & 1.33 & 68.78 & 0.89 \\ 

\textit{2} & 0.021   & 0.070   & 35.34 & 0.93/0.89 & 27.35 & 1.34 & 67.58 & 0.90 \\ 

%\textit{3*} & 0.018 & 0.0061  & 33.22 & 0.95/0.91 & 27.99 & 1.28 & 64.89 & 0.92 \\ 
\textit{3} & 0.018 & 0.0061  & 33.22 & 0.95/0.91 & 27.99 & 1.28 & 64.89 & 0.92 \\ 

\textit{4} & 0.017   & 0.058   & 31.89 & 0.95/0.92 & 28.56 & 1.24 & 64.82 & 0.92 \\ 

\textit{5} & 0.017   & 0.051   & 30.69 & 0.96/0.92 & 28.83 & 1.21 & 65.15 & 0.92 \\ 

\textit{6} &   0.016  &  0.050   &  31.17 &  0.96/0.92  &  29.04 & 1.19  & 64.86 & 0.92   \\ 


\specialrule{.15em}{.05em}{.05em}
 %\multicolumn{8}{l}{\multirow{1}{*}{\small{(*: equals to the full model used in this paper)}}}

\end{tabular}  
}

	%\vspace{-0.2cm}
\caption{Ablations on input source view numbers ($N$), tested on \texttt{DFDC} dataset (1807 testing samples for reconstruction task, 200 testing pairs for animation), with mean results reported and best ones bolded. $\downarrow$ ($\uparrow$) denotes that lower (higher) is better. 
}

\label{tab: num_refs_all}
\end{wraptable}

==> sub/tab/test_wrap_tab3.tex <==

\begin{wraptable}{r}{0.7\textwidth}

\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{0.9\linewidth}{!}{
%\hspace{-1cm}
\begin{tabular}{ccccccccc}
\specialrule{.15em}{.05em}{.05em}
%\hline
 
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{\textit{Model}}}} & \multicolumn{6}{c}{\multirow{1}{*}{\textbf{\textit{Reconstruction}}}} & \multicolumn{2}{c}{\multirow{1}{*}{\textbf{\textit{Animation}}}} \\

\cmidrule(lr){2-7}
\cmidrule(lr){8-9}

 & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{L1} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{LPIPS} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{MS-/SSIM} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{PSNR} ($\uparrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{AKD} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{FID} ($\downarrow$)}} & \multicolumn{1}{c}{\multirow{1}{*}{\texttt{CSIM} ($\uparrow$)}}\\

\specialrule{.08em}{.05em}{.05em}
%\hline



\textit{Full (\texttt{SLIDE})} & {\bf{0.018}}  & {\bf{0.0061}} & {\bf{33.22}} & {\bf{0.95}}/{\bf{0.91}} & 27.99 & {\bf{1.28}} & {\bf{64.89}} & {\bf{0.92}} \\  

\textit{w/o Mot. Evol.} & 0.022  & 0.082   & 42.47 & 0.93/0.87 & {\bf{28.60}} & 1.53 & 71.88 & 0.88  \\ 

\textit{w/o App.  Assist.} & 0.024   & 0.085   & 41.89 & 0.92/0.85 & 27.88 & 1.29 & 75.35 & 0.90  \\ 

\textit{w/o Mult. Fus.} & 0.032   & 0.108   & 54.57 & 0.88/0.84 & 24.24 & 1.78 & 80.34 & 0.89  \\ 


\specialrule{.15em}{.05em}{.05em} 
\end{tabular}
}


%\vspace{-0.2cm}
\caption{Ablations results of \texttt{SLIDE} on \texttt{DFDC} dataset (1807 testing samples for reconstruction task, 200 testing pairs for animation), with mean results reported and best ones bolded. $\downarrow$ ($\uparrow$) denotes that lower (higher) is better.
}

\label{tab: ablations}
\end{wraptable}
